Local Effects of Grid-Forming Converters Providing Frequency Regulation to Bulk Power Grids

The progressive displacing of conventional generation in favour of renewable energy sources requires restoring an adequate capacity of regulating power to ensure reliable operation of power systems. Battery Energy Storage Systems (BESSs) are considered to be promising assets to restore suitable frequency regulation capacity levels. BESSs are typically connected to the grid with power-converters, able to operate in either grid-forming or grid-following modes. This paper quantitatively assesses the impact on the local distribution grid of BESSs providing frequency regulation to bulk power systems. Specific metrics are proposed to compare the performance of grid-forming and grid-following control. Experimental results are obtained taking advantage of a 720 kVA/500 kWh BESS connected to the 20 kV distribution grid of the EPFL campus. The quantitative evaluation based on suitably proposed metrics confirms the superior performance of the grid-forming strategy, compared to the grid-following one.

==> ISGT ASIA 2021/authors.tex <==
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
% Title of the Paper
%\title{Effect of Grid-Forming Converters-Interfaced Battery Storage Systems Providing Frequency Regulation in Bulk Power Grids}
\title{Local Effects of Grid-Forming Converters Providing Frequency Regulation \\ to Bulk Power Grids}


% Author names and affiliations
\author{
%\IEEEauthorblockN{Antonio Zecchino}
%\IEEEauthorblockA{SwissGrid AG \\
%Ancillary Services \& Analytics \\
%Aarau, Aargau, Switzerland\\
%antonio.zecchino@epfl.ch
%}
%\and
\IEEEauthorblockN{Antonio Zecchino, Francesco Gerini, Yihui Zuo, \\Rachid Cherkaoui, Mario Paolone}
\IEEEauthorblockA{Distributed Electrical Systems Laboratory (DESL)\\
Ecole Polytechnique Fédérale de Lausanne, EPFL\\
Lausanne, Switzerland\\
\{antonio.zecchino, francesco.gerini, yihui.zuo,\\ rachid.cherkaoui, mario.paolone\}@epfl.ch}
\and
\IEEEauthorblockN{Elena Vagnoni}
\IEEEauthorblockA{Technology Platform for Hydraulic Machines \\ 
Ecole Polytechnique Fédérale de Lausanne, EPFL\\
Lausanne, Switzerland\\
\{elena.vagnoni\}@epfl.ch}
\thanks{{This work is supported by OSMOSE project.  The project has received funding from the European Union's Horizon 2020 Research and Innovation Program under Grant 773406.}}

}



==> ISGT ASIA 2021/user.tex <==
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
%\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}

%	##########
%	Packages
%	##########

%	Citations
%\usepackage{cite} % Sort and compress reference ranges.
%	Figures
\usepackage[caption=false,font=footnotesize]{subfig}	%	The option 'caption=false' is required to keep IEEE-style captions.
\usepackage{graphicx}
%	Math
\usepackage{amsmath,amsfonts,amssymb,amsthm}
\usepackage{mathtools}
\usepackage{mathrsfs}	%	mathscr
\usepackage{subdepth}	%	uniform subscript position
%	Alignment
\usepackage{array}	%	better appearance for array and tabular environments
\usepackage[inline]{enumitem} % enumerate stuff in line
%	References, Hyperlinks, etc.
\usepackage{hyperref}
\usepackage[sort,compress,capitalise]{cleveref}	%	...
\usepackage{url}
%	Miscellaneous
\usepackage{xcolor} % Coloured text
\usepackage{xspace} % Intelligent spacing (acronym commands) 
\usepackage{lipsum}
%	Draw
\usepackage{tikz}
\usetikzlibrary{babel}  % Avoid problems due to babel library
\usepackage[straightvoltages,nooldvoltagedirection]{circuitikz}
\usetikzlibrary{shapes,arrows}
\usepackage{verbatim}
\usepackage{multirow}
% Other
\usepackage[utf8]{inputenc}
\usepackage{fourier} 
\usepackage{array}
\usepackage{makecell}



